Can Nonstandard Neutrino Interactions explain the XENON1T spectral excess?

We perform a constrained spectral fit analysis of the excess observed in the electron recoil energy spectrum by XENON1T with neutrino magnetic moment, charge radius, neutrino millicharge and new light vector and scalar mediators. Within the limits allowed by other laboratory experiments we find that the excess can be explained in the range$\ (2-4)\times 10^{-11}\mu _{B} $ for the magnetic moment,$\ (2-6)\times 10^{-31}$cm$^{2}$ for the charge radius, $\ (1.7-2.3)\times 10^{-12}e$ for the millicharge and $(10-100)\ $keV masses of light mediators with couplings of $ 3.5\times 10^{-7}$ for vector/axial-vector, $1\times 10^{-6}$ and $4\times 10^{-6}$ for scalar and pseudo-scalar mediators respectively. Among all neutrino millicharge, magnetic moment and vector mediators fit better to the observed spectrum. We also derive constraints on all new physics parameters considered here.

==> biblio.tex <==
@article{Fujikawa:1980yx,
    author = "Fujikawa, Kazuo and Shrock, Robert",
    title = "{The Magnetic Moment of a Massive Neutrino and Neutrino Spin Rotation}",
    reportNumber = "ITP-SB-80-38",
    doi = "10.1103/PhysRevLett.45.963",
    journal = "Phys. Rev. Lett.",
    volume = "45",
    pages = "963",
    year = "1980"
}
    @article{Vogel:1989iv,
    author = "Vogel, P. and Engel, J.",
    title = "{Neutrino Electromagnetic Form-Factors}",
    reportNumber = "CALT-63-539",
    doi = "10.1103/PhysRevD.39.3378",
    journal = "Phys. Rev. D",
    volume = "39",
    pages = "3378",
    year = "1989"
}
@article{Dvornikov:2003js,
    author = "Dvornikov, Maxim and Studenikin, Alexander",
    title = "{Electric charge and magnetic moment of massive neutrino}",
    eprint = "hep-ph/0305206",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.69.073001",
    journal = "Phys. Rev. D",
    volume = "69",
    pages = "073001",
    year = "2004"
}
@article{Dvornikov:2004sj,
    author = "Dvornikov, Maxim S. and Studenikin, Alexander I.",
    title = "{Electromagnetic form-factors of a massive neutrino}",
    eprint = "hep-ph/0411085",
    archivePrefix = "arXiv",
    doi = "10.1134/1.1800181",
    journal = "J. Exp. Theor. Phys.",
    volume = "99",
    pages = "254--269",
    year = "2004"
}
@article{Aprile:2020tmw,
    author = "Aprile, E. and others",
    collaboration = "XENON",
    title = "{Observation of Excess Electronic Recoil Events in XENON1T}",
    eprint = "2006.09721",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    month = "6",
    year = "2020"
}
@article{Aprile:2020yad,
    author = "Aprile, E. and others",
    collaboration = "XENON",
    title = "{Energy resolution and linearity in the keV to MeV range measured in XENON1T}",
    eprint = "2003.03825",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "3",
    year = "2020"
}
@article{shokley:slides,
    author = "Evan Shockley",
    title  =  "{Search for New Physics with Electronic-Recoil Events in XENON1T}", 
    journal = "https://www.dropbox.com/s/vrq49tldjdfvnjh\\/shockley20200617.pdf?dl=0",
    year   =  "June 17th, 2020"
}
@article{Bahcall:2004mz,
    author = "Bahcall, John N. and Pena-Garay, Carlos",
    title = "{Solar models and solar neutrino oscillations}",
    eprint = "hep-ph/0404061",
    archivePrefix = "arXiv",
    doi = "10.1088/1367-2630/6/1/063",
    journal = "New J. Phys.",
    volume = "6",
    pages = "63",
    year = "2004"
}
@article{Zyla:PDG2020,
    author = "P.A. Zyla et al.",
    collaboration = "Particle Data Group", 
    journal = "to be published in Prog. Theor. Exp. Phys. 2020, 083C01 (2020)",
}
@article{Lopes:2013nfa,
    author = "Lopes, Ilídio and Turck-Chièze, Sylvaine",
    title = "{Solar neutrino physics oscillations: Sensitivity to the electronic density in the Sun's core}",
    eprint = "1302.2791",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.SR",
    doi = "10.1088/0004-637X/765/1/14",
    journal = "Astrophys. J.",
    volume = "765",
    pages = "14",
    year = "2013"
}
@article{Borexino:2017fbd,
    author = "Agostini, M. and others",
    collaboration = "Borexino",
    title = "{Limiting neutrino magnetic moments with Borexino Phase-II solar neutrino data}",
    eprint = "1707.09355",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    doi = "10.1103/PhysRevD.96.091103",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "9",
    pages = "091103",
    year = "2017"
}
@article{Khan:2017djo,
    author = "Khan, Amir N.",
    title = "{$\sin ^{2}\theta _{W}$ Estimate and Neutrino Electromagnetic Properties from Low-Energy Solar Data}",
    eprint = "1709.02930",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-18-444-ND-T",
    doi = "10.1088/1361-6471/ab0057",
    journal = "J. Phys. G",
    volume = "46",
    number = "3",
    pages = "035005",
    year = "2019"
}
@article{Khan:2019cvi,
    author = "Khan, Amir N. and Rodejohann, Werner",
    title = "{New physics from COHERENT data with an improved quenching factor}",
    eprint = "1907.12444",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-19-426-T",
    doi = "10.1103/PhysRevD.100.113003",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "11",
    pages = "113003",
    year = "2019"
}
@article{Boehm:2020ltd,
    author = "Boehm, Celine and Cerdeno, David G. and Fairbairn, Malcolm and Machado, Pedro A.N. and Vincent, Aaron C.",
    title = "{Light new physics in XENON1T}",
    eprint = "2006.11250",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-20-247-T, IFT-UAM/CSIC-20-88",
    month = "6",
    year = "2020"
}
@article{Kannike:2020agf,
    author = "Kannike, Kristjan and Raidal, Martti and Veermäe, Hardi and Strumia, Alessandro and Teresi, Daniele",
    title = "{Dark Matter and the XENON1T electron recoil excess}",
    eprint = "2006.10735",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Takahashi:2020bpq,
    author = "Takahashi, Fuminobu and Yamada, Masaki and Yin, Wen",
    title = "{XENON1T anomaly from anomaly-free ALP dark matter and its implications for stellar cooling anomaly}",
    eprint = "2006.10035",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "TU-1104, IPMU20-0069",
    month = "6",
    year = "2020"
}
@article{Lindner:2018kjo,
    author = "Lindner, Manfred and Queiroz, Farinaldo S. and Rodejohann, Werner and Xu, Xun-Jie",
    title = "{Neutrino-electron scattering: general constraints on Z$^{′}$ and dark photon models}",
    eprint = "1803.00060",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IIPDM-2018-02",
    doi = "10.1007/JHEP05(2018)098",
    journal = "JHEP",
    volume = "05",
    pages = "098",
    year = "2018"
}
@article{Arcadi:2018xdd,
    author = "Arcadi, Giorgio and Heeck, Julian and Heizmann, Florian and Mertens, Susanne and Queiroz, Farinaldo S. and Rodejohann, Werner and Slezák, Martin and Valerius, Kathrin",
    title = "{Tritium beta decay with additional emission of new light bosons}",
    eprint = "1811.03530",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ULB-TH/18-12, UCI-TR-2018-14",
    doi = "10.1007/JHEP01(2019)206",
    journal = "JHEP",
    volume = "01",
    pages = "206",
    year = "2019"
}
@article{Erler:2004in,
    author = "Erler, Jens and Ramsey-Musolf, Michael J.",
    title = "{The Weak mixing angle at low energies}",
    eprint = "hep-ph/0409169",
    archivePrefix = "arXiv",
    reportNumber = "FT-2004-03, CALTECH-MAP-300",
    doi = "10.1103/PhysRevD.72.073003",
    journal = "Phys. Rev. D",
    volume = "72",
    pages = "073003",
    year = "2005"
}
@article{Cadeddu:2020lky,
    author = "Cadeddu, M. and Dordei, F. and Giunti, C. and Li, Y.F. and Picciau, E. and Zhang, Y.Y.",
    title = "{Physics results from the first COHERENT observation of CE$\nu$NS in argon and their combination with cesium-iodide data}",
    eprint = "2005.01645",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "5",
    year = "2020"
}
@article{Deniz:2009mu,
    author = "Deniz, M. and others",
    collaboration = "TEXONO",
    title = "{Measurement of Nu(e)-bar -Electron Scattering Cross-Section with a CsI(Tl) Scintillating Crystal Array at the Kuo-Sheng Nuclear Power Reactor}",
    eprint = "0911.1597",
    archivePrefix = "arXiv",
    primaryClass = "hep-ex",
    reportNumber = "AS-TEXONO-09-04",
    doi = "10.1103/PhysRevD.81.072001",
    journal = "Phys. Rev. D",
    volume = "81",
    pages = "072001",
    year = "2010"
}
@article{Giunti:2015gga,
    author = "Giunti, Carlo and Kouzakov, Konstantin A. and Li, Yu-Feng and Lokhov, Alexey V. and Studenikin, Alexander I. and Zhou, Shun",
    title = "{Electromagnetic neutrinos in laboratory experiments and astrophysics}",
    eprint = "1506.05387",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1002/andp.201500211",
    journal = "Annalen Phys.",
    volume = "528",
    pages = "198--215",
    year = "2016"
}
@proceedings{Dev:2019anc,
    author = "Bhupal Dev, P.S. and others",
    title = "{Neutrino Non-Standard Interactions: A Status Report}",
    eprint = "1907.00991",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-CONF-19-299-T",
    doi = "10.21468/SciPostPhysProc.2.001",
    volume = "2",
    pages = "001",
    year = "2019"
}
@article{NovalesSanchez:2008tn,
    author = "Novales-Sanchez, H. and Rosado, A. and Santiago-Olan, V. and Toscano, J.J.",
    title = "{Effects of physics beyond the standard model on the neutrino charge radius: an effective Lagrangian approach}",
    eprint = "0805.4177",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.78.073014",
    journal = "Phys. Rev. D",
    volume = "78",
    pages = "073014",
    year = "2008"
}
@article{Bell:2006wi,
    author = "Bell, Nicole F. and Gorchtein, Mikhail and Ramsey-Musolf, Michael J. and Vogel, Petr and Wang, Peng",
    title = "{Model independent bounds on magnetic moments of Majorana neutrinos}",
    eprint = "hep-ph/0606248",
    archivePrefix = "arXiv",
    reportNumber = "CALT-68-2603, KRL-MAP-321",
    doi = "10.1016/j.physletb.2006.09.055",
    journal = "Phys. Lett. B",
    volume = "642",
    pages = "377--383",
    year = "2006"
}
@article{Bell:2005kz,
    author = "Bell, Nicole F. and Cirigliano, Vincenzo and Ramsey-Musolf, Michael J. and Vogel, Petr and Wise, Mark B.",
    title = "{How magnetic is the Dirac neutrino?}",
    eprint = "hep-ph/0504134",
    archivePrefix = "arXiv",
    reportNumber = "CALT-08-2554, KRL-MAP-307",
    doi = "10.1103/PhysRevLett.95.151802",
    journal = "Phys. Rev. Lett.",
    volume = "95",
    pages = "151802",
    year = "2005"
}
@article{Musolf:1990sa,
    author = "Musolf, M.J. and Holstein, Barry R.",
    title = "{Observability of the anapole moment and neutrino charge radius}",
    reportNumber = "MIT-CTP-1896",
    doi = "10.1103/PhysRevD.43.2956",
    journal = "Phys. Rev. D",
    volume = "43",
    pages = "2956--2970",
    year = "1991"
}
@article{Babu:2019iml,
    author = "Babu, K.S. and Chauhan, Garv and Bhupal Dev, P.S.",
    title = "{Neutrino Non-Standard Interactions via Light Scalars in the Earth, Sun, Supernovae and the Early Universe}",
    eprint = "1912.13488",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "OSU-HEP-19-11",
    doi = "10.1103/PhysRevD.101.095029",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "9",
    pages = "095029",
    year = "2020"
}
@article{Cerdeno:2016sfi,
    author = "Cerdeño, David G. and Fairbairn, Malcolm and Jubb, Thomas and Machado, Pedro A. N. and Vincent, Aaron C. and B\oe hm, Céline",
    title = "{Physics from solar neutrinos in dark matter direct detection experiments}",
    eprint = "1604.01025",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IFT-UAM-CSIC-16-031, FTUAM-16-12, IPPP-16-27, DCTP-16-54, KCL-PH-TH-2016-19",
    doi = "10.1007/JHEP09(2016)048",
    journal = "JHEP",
    volume = "05",
    pages = "118",
    year = "2016",
    note = "[Erratum: JHEP 09, 048 (2016)]"
}
@article{AristizabalSierra:2020edu,
    author = "Aristizabal Sierra, D. and De Romeri, V. and Flores, L.J. and Papoulias, D.K.",
    title = "{Light vector mediators facing XENON1T data}",
    eprint = "2006.12457",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Miranda:2020kwy,
    author = "Miranda, O.G. and Papoulias, D.K. and Tórtola, M. and Valle, J.W.F.",
    title = "{XENON1T signal from transition neutrino magnetic moments}",
    eprint = "2007.01765",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "7",
    year = "2020"
}
@article{Okada:2020evk,
    author = "Okada, Nobuchika and Okada, Satomi and Raut, Digesh and Shafi, Qaisar",
    title = "{Dark Matter $Z^\prime$ and XENON1T Excess from $U(1)_X$ Extended Standard Model}",
    eprint = "2007.02898",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "7",
    year = "2020"
}
@article{Ge:2020jfn,
    author = "Ge, Shao-Feng and Pasquini, Pedro and Sheng, Jie",
    title = "{Solar Neutrino Scattering with Electron into Massive Sterile Neutrino}",
    eprint = "2006.16069",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Lindner:2020kko,
    author = "Lindner, Manfred and Mambrini, Yann and de Melo, Tessio B. and Queiroz, Farinaldo S.",
    title = "{XENON1T Anomaly: A Light $Z^\prime$}",
    eprint = "2006.14590",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IIP-2020",
    month = "6",
    year = "2020"
}
@article{Bally:2020yid,
    author = "Bally, Andreas and Jana, Sudip and Trautner, Andreas",
    title = "{Neutrino self-interactions and XENON1T electron recoil excess}",
    eprint = "2006.11919",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Alonso-Alvarez:2020cdv,
    author = "Alonso-Álvarez, G. and Ertas, F. and Jaeckel, J. and Kahlhoefer, F. and Thormaehlen, L.J.",
    title = "{Hidden Photon Dark Matter in the Light of XENON1T and Stellar Cooling}",
    eprint = "2006.11243",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Chala:2020pbn,
    author = "Chala, Mikael and Titov, Arsenii",
    title = "{One-loop running of dimension-six Higgs-neutrino operators and implications of a large neutrino dipole moment}",
    eprint = "2006.14596",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Amaral:2020tga,
    author = "Amaral, Dorian Warren Praia, do. and Cerdeno, David G. and Foldenauer, Patrick and Reid, Elliott",
    title = "{Solar neutrino probes of the muon anomalous magnetic moment in the gauged $U(1)_{L_\mu-L_\tau}$}",
    eprint = "2006.11225",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPPP/20/24, IFT-UAM/CSIC-20-70",
    month = "6",
    year = "2020"
}
@article{Coloma:2020voz,
    author = "Coloma, Pilar and Huber, Patrick and Link, Jonathan M.",
    title = "{Telling Solar Neutrinos from Solar Axions When You Can't Shut Off the Sun}",
    eprint = "2006.15767",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Benakli:2020vng,
    author = "Benakli, Karim and Branchina, Carlo and Lafforgue-Marmet, Gaëtan",
    title = "{U(1) mixing and the Weak Gravity Conjecture}",
    eprint = "2007.02655",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "7",
    year = "2020"
}
@article{Chigusa:2020bgq,
    author = "Chigusa, So and Endo, Motoi and Kohri, Kazunori",
    title = "{Constraints on electron-scattering interpretation of XENON1T excess}",
    eprint = "2007.01663",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KEK-TH-2236, KEK-Cosmo-258",
    month = "7",
    year = "2020"
}
@article{Li:2020naa,
    author = "Li, Tianjun",
    title = "{The KSVZ Axion and Pseudo-Nambu-Goldstone Boson Models for the XENON1T Excess}",
    eprint = "2007.00874",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "7",
    year = "2020"
}
@article{Baek:2020owl, 
    author = "Baek, Seungwon and Kim, Jongkuk and Ko, P.",
    title = "{XENON1T excess in local $Z_2$ DM models with light dark sector}",
    eprint = "2006.16876",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Gao:2020wfr,
    author = "Gao, Yu and Li, Tianjun",
    title = "{Lepton Number Violating Electron Recoils at XENON1T by the $U(1)_{B-L}$ Model with Non-Standard Interactions}",
    eprint = "2006.16192",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Ko:2020gdg,
    author = "Ko, P. and Tang, Yong",
    title = "{Semi-annihilating $Z_3$ Dark Matter for XENON1T Excess}",
    eprint = "2006.15822",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{An:2020tcg,
    author = "An, Haipeng and Yang, Daneng",
    title = "{Direct detection of freeze-in inelastic dark matter}",
    eprint = "2006.15672",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{McKeen:2020vpf,
    author = "McKeen, David and Pospelov, Maxim and Raj, Nirmal",
    title = "{Hydrogen portal to exotic radioactivity}",
    eprint = "2006.15140",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Bloch:2020uzh,
    author = "Bloch, Itay M. and Caputo, Andrea and Essig, Rouven and Redigolo, Diego and Sholapurkar, Mukul and Volansky, Tomer",
    title = "{Exploring New Physics with O(keV) Electron Recoils in Direct Detection Experiments}",
    eprint = "2006.14521",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Budnik:2020nwz,
    author = "Budnik, Ranny and Kim, Hyungjin and Matsedonskyi, Oleksii and Perez, Gilad and Soreq, Yotam",
    title = "{Probing the relaxed relaxion and Higgs-portal with S1 \& S2}",
    eprint = "2006.14568",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Smirnov:2020zwf,
    author = "Smirnov, Juri and Beacom, John F.",
    title = "{Co-SIMP Miracle}",
    eprint = "2002.04038",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "2",
    year = "2020"
}
@article{Jho:2020sku,
    author = "Jho, Yongsoo and Park, Jong-Chul and Park, Seong Chan and Tseng, Po-Yan",
    title = "{Gauged Lepton Number and Cosmic-ray Boosted Dark Matter for the XENON1T Excess}",
    eprint = "2006.13910",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Bramante:2020zos,
    author = "Bramante, Joseph and Song, Ningqiang",
    title = "{Electric But Not Eclectic: Thermal Relic Dark Matter for the XENON1T Excess}",
    eprint = "2006.14089",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Zu:2020idx,
    author = "Zu, Lei and Yuan, Guan-Wen and Feng, Lei and Fan, Yi-Zhong",
    title = "{Mirror Dark Matter and Electronic Recoil Events in XENON1T}",
    eprint = "2006.14577",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Fornal:2020npv,
    author = "Fornal, Bartosz and Sandick, Pearl and Shu, Jing and Su, Meng and Zhao, Yue",
    title = "{Boosted Dark Matter Interpretation of the XENON1T Excess}",
    eprint = "2006.11264",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "6",
    year = "2020"
}
@article{Rosado:1999yn,
      author         = "Rosado, A.",
      title          = "{Physical electroweak anapole moment for the neutrino}",
      journal        = "Phys. Rev.",
      volume         = "D61",
      year           = "2000",
      pages          = "013001",
      doi            = "10.1103/PhysRevD.61.013001",
      SLACcitation   = "%%CITATION = PHRVA,D61,013001;%%"
}
@article{Arcadi:2020zni,
    author = "Arcadi, Giorgio and Bally, Andreas and Goertz, Florian and Tame-Narvaez, Karla and Tenorth, Valentin and Vogl, Stefan",
    title = "{EFT Interpretation of XENON1T Electron Recoil Excess: Neutrinos and Dark Matter}",
    eprint = "2007.08500",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "7",
    year = "2020"
}
@article{Harnik:2012ni,
    author = "Harnik, Roni and Kopp, Joachim and Machado, Pedro A.N.",
    title = "{Exploring nu Signals in Dark Matter Detectors}",
    eprint = "1202.6073",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-12-048-T",
    doi = "10.1088/1475-7516/2012/07/026",
    journal = "JCAP",
    volume = "07",
    pages = "026",
    year = "2012"
}
}
@article{Aalseth:2017fik,
    author = "Aalseth, C.E. and others",
    title = "{DarkSide-20k: A 20 tonne two-phase LAr TPC for direct dark matter detection at LNGS}",
    eprint = "1707.08145",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    reportNumber = "FERMILAB-PUB-17-298-PPD",
    doi = "10.1140/epjp/i2018-11973-4",
    journal = "Eur. Phys. J. Plus",
    volume = "133",
    pages = "131",
    year = "2018"
}
@article{Aalbers:2016jon,
    author = "Aalbers, J. and others",
    collaboration = "DARWIN",
    title = "{DARWIN: towards the ultimate dark matter detector}",
    eprint = "1606.07001",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1088/1475-7516/2016/11/017",
    journal = "JCAP",
    volume = "11",
    pages = "017",
    year = "2016"
}
@article{Aalbers:2020gsn,
    author = "Aalbers, J. and others",
    collaboration = "DARWIN",
    title = "{Solar Neutrino Detection Sensitivity in DARWIN via Electron Scattering}",
    eprint = "2006.03114",
    archivePrefix = "arXiv",
    primaryClass = "physics.ins-det",
    month = "6",
    year = "2020"
}
@article{Raffelt:1999gv,
    author = "Raffelt, G.G.",
    title = "{Limits on neutrino electromagnetic properties: An update}",
    doi = "10.1016/S0370-1573(99)00074-5",
    journal = "Phys. Rept.",
    volume = "320",
    pages = "319--327",
    year = "1999"
}
@article{Davidson:2000hf,
    author = "Davidson, Sacha and Hannestad, Steen and Raffelt, Georg",
    title = "{Updated bounds on millicharged particles}",
    eprint = "hep-ph/0001179",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-99-384",
    doi = "10.1088/1126-6708/2000/05/003",
    journal = "JHEP",
    volume = "05",
    pages = "003",
    year = "2000"
}
